Rhetoric, Logic, and Dialectic: Advancing Theory-based Argument Quality Assessment in Natural Language Processing

Though preceding work in computational argument quality (AQ) mostly focuses on assessing overall AQ, researchers agree that writers would benefit from feedback targeting individual dimensions of argumentation theory. However, a large-scale theory-based corpus and corresponding computational models are missing. We fill this gap by conducting an extensive analysis covering three diverse domains of online argumentative writing and presenting GAQCorpus: the first large-scale English multi-domain (community Q&A forums, debate forums, review forums) corpus annotated with theory-based AQ scores. We then propose the first computational approaches to theory-based assessment, which can serve as strong baselines for future work. We demonstrate the feasibility of large-scale AQ annotation, show that exploiting relations between dimensions yields performance improvements, and explore the synergies between theory-based prediction and practical AQ assessment.

==> experiments-old.tex <==
\section{Experiments}
\label{sec:experiments}
In the remainder of the paper, we employ the proposed architectures to answer the following research questions:
    (\textbf{Q1}): \emph{Can the interrelations between the different AQ dimensions suggested by the taxonomy be exploited in a computational setup?}
(\textbf{Q2}): \emph{How well does the corpus support training DL models for multi-domain evaluation?}
(\textbf{Q3}): \emph{Dagstuhl research question}
(\textbf{Q4}): \emph{What are concrete scenarios in which combining theory-based and practical AQ assessment can result in synergies?}

\subsection{Experiments on \corpus}
In order to answer Q1, and Q2, and to provide strong baselines for future theory-based AQ research, we first run experiments on \corpus.

\paragraph{Experimental Setup}
%% training setup and data
We run the experiments on \corpus in two main training settings: (1) \emph{in-domain}, in which we train on the domain-specific training sets only, and (2) \emph{all-domains}, in which we join the training sets across all domains. This way, we obtain a larger and more diverse training set. The training, development, and test portions correspond to the ones presented in Section $2$. Consequently, for each domain and each argument quality dimension, we have three different test annotations on the same instances against which we evaluate our models.
%% baselines
We compare our approach against the following baselines:\jttodo{looking at Sec 3, I wonder if should just merge the models below in with that section?  It's not like we made a new DL model for argumentation and it fits together nicely.  So Sec 3 could just be called Models.  Just a thought.}

\vspace{0.5em}
\noindent \textsc{Arg length}: To obtain an estimate of the difficulty of the task(s) and to measure potential bias regarding argument length in our data set, we count the number of characters in the argument and correlate it against the test scores.\jttodo{why characters instead of words?}

\vspace{0.4em}
\noindent \textsc{SVR$_{tfidf}$}: We run a simple Support Vector Regression (SVR) with tf-idf feature vectors.\jttodo{which toolkit}

\vspace{0.4em}
\noindent \textsc{SVR$_{embd}$}: For each word in the argument, we lookup its fastText\cite{Bojanowski:2017tacl} embedding\footnote{\url{https://dl.fbaipublicfiles.com/fasttext/vectors-english/wiki-news-300d-1M-subword.vec.zip}} representations and average over all embeddings to represent the whole argument and feed it into an SVR.

\vspace{0.4em}
\noindent \textsc{Wachsmuth$_{All}$}: Further, we replicate the approach of \newcite{wachsmuth-etal-2016-using}, who employ a rich set of features including standard features (e.g., token n-grams, part-of-speech tags, etc.) as well as higher-level features (e.g., sentiment flows, argumentative discourse units etc.), which they then use as input for an SVR. For this variant of the approach, we employ all features.

\vspace{0.4em}
\noindent \textsc{Wachsmuth$_{CFS}$}: For the second variant, we run correlation-based feature selection on the training set and employ only the features which were found to be the most predictive.
%
\vspace{0.5em}

We optimize the hyperparameters of all models on the development set portions. For the SVR, we grid search in $c \in \{0.001, 0.01, 0.1, 1.0, 10\}$ and $\epsilon \in \{0.001, 0.01, 0.1, 1.0\}$. For the BERT-based models, we optimize the learning rate $\lambda \in \{2e-5, 3e-5\}$ and the number of training epochs $\in \{3,4\}$.
\paragraph{Results.}\jttodo{let's make this a subsection}
%
%
The respective Pearson correlation scores for the four argument quality dimensions on the three different test sets per domain can be seen in Table \ref{tbl:in-domains}.
%
\setlength{\tabcolsep}{4pt}
\begin{table*}[t]\centering
\small
\begin{tabular}{llrrrrrrrrrr}\toprule
 &\textbf{} &\multicolumn{3}{c}{\textbf{QA forums}} &\multicolumn{3}{c}{\textbf{Debate Forums}} &\multicolumn{3}{c}{\textbf{Review Forums}} \\\cmidrule{3-11}
&\textbf{Model} &\textbf{Crowd} &\textbf{Expert} &\textbf{Mix} &\textbf{Crowd} &\textbf{Expert} &\textbf{Mix} &\textbf{Crowd} &\textbf{Expert} &\textbf{Mix} \\\midrule
\multirow{7}{*}{\textbf{Overall}} &\textbf{\textsc{Arg length}} &0.498 &0.236 &0.406 &0.542 &0.232 &0.420 &0.486 &0.190 &0.365 \\
&\textbf{\textsc{Wachsmuth$_{All}$}} &0.331 &0.224 &0.307 &0.341 &0.176 &0.284 &0.481 &0.188 &0.360 \\
&\textbf{\textsc{Wachsmuth$_{CFS}$}} &0.550 &0.340 &0.492 &0.524 &0.264 &0.432 &\textbf{0.619} &0.342 &0.533 \\
&\textbf{\textsc{SVR$_{tfidf}$}} &0.381 &0.323 &0.389 &0.299 &0.179 &0.265 &0.446 &0.340 &0.450 \\
&\textbf{\textsc{SVR$_{embd}$}} &0.323 &0.180 &0.278 &0.467 &0.239 &0.388 &0.223 &0.227 &0.265 \\
&\textbf{\textsc{BERT ST}} &\textbf{0.681} &0.498 &0.652 &0.575 &0.346 &0.511 &0.611 &0.450 &\textbf{0.605} \\
&\textbf{\textsc{BERT MT$_{flat}$}} &0.671 &\textbf{0.535} &\textbf{0.667} &\textbf{0.607} &\textbf{0.362} &\textbf{0.537} &0.534 &\textbf{0.478} &0.588 \\
&\textbf{\textbf{\textsc{BERT MT$_{hier}$}}}  &0.668 &0.528 &0.661 &0.480 &0.393 &0.494 &0.563 &0.465 &0.593 \\
\midrule
\multirow{7}{*}{\textbf{Cogency}} & \textbf{\textsc{Arg length}} &0.502 &0.227 &0.420 &0.574 &0.225 &0.437 &0.491 &0.125 &0.340 \\ &\textbf{\textsc{Wachsmuth$_{All}$}}  &0.291 &0.161 &0.259 &0.278 &0.120 &0.219 &0.493 &0.043 &0.287 \\
&\textbf{\textsc{Wachsmuth$_{CFS}$}} &0.565 &0.311 &0.503 &0.548 &0.232 &0.429 &0.611 &0.223 &0.464 \\
&\textbf{\textsc{SVR$_{tfidf}$}} &0.449 &0.330 &0.444 &0.295 &0.164 &0.257 &0.409 &0.264 &0.384 \\
&\textbf{\textsc{SVR$_{embd}$}} &0.301 &0.154 &0.261 &0.404 &0.196 &0.333 &0.264 &-0.059 &0.103 \\
&\textbf{\textsc{BERT ST}} &0.623 &0.405 &0.587 &0.556 &0.337 &0.503 &\textbf{0.618} &0.359 &0.554 \\
&\textbf{\textsc{BERT MT$_{flat}$}} &\textbf{0.651} &0.457 &0.633 &\textbf{0.622} &0.343 &\textbf{0.541} &0.533 &\textbf{0.440} &\textbf{0.561} \\
&\textbf{\textbf{\textsc{BERT MT$_{hier}$}}}  &0.650 &\textbf{0.468} &\textbf{0.638} &0.476 &\textbf{0.353} &0.474 &0.559 &0.388 &0.541 \\
\midrule
\multirow{7}{*}{\textbf{Effectiveness}} & \textbf{\textsc{Arg length}} &0.475 &0.237 &0.390 &0.502 &0.225 &0.399 &0.425 &0.251 &0.372 \\ &\textbf{\textsc{Wachsmuth$_{All}$}}  &0.333 &0.203 &0.295 &0.274 &0.194 &0.265 &0.471 &0.171 &0.336 \\
&\textbf{\textsc{Wachsmuth$_{CFS}$}} &0.555 &0.393 &0.523 &0.528 &0.281 &0.450 &0.567 &0.246 &0.432 \\
&\textbf{\textsc{SVR$_{tfidf}$}} &0.432 &0.313 &0.411 &0.141 &0.074 &0.120 &0.354 &0.253 &0.340 \\
&\textbf{\textsc{SVR$_{embd}$}} &0.328 &0.204 &0.293 &0.456 &0.264 &0.403 &0.186 &0.144 &0.187 \\
&\textbf{\textsc{BERT ST}} &0.596 &0.509 &0.612 &0.548 &0.405 &0.542 &\textbf{0.639} &0.370 &\textbf{0.555} \\
&\textbf{\textsc{BERT MT$_{flat}$}} &\textbf{0.663} &0.549 &\textbf{0.671} &\textbf{0.599} &0.408 &\textbf{0.570} &0.522 &\textbf{0.389} &0.514 \\
&\textbf{\textbf{\textsc{BERT MT$_{hier}$}}}  &0.656 &\textbf{0.552} &0.670 &0.477 &\textbf{0.443} &0.532 &0.466 &0.388 &0.486 \\
\midrule
\multirow{7}{*}{\textbf{Reasonableness}} & \textbf{\textsc{Arg length}} &0.480 &0.245 &0.396 &0.535 &0.170 &0.377 &0.496 &0.241 &0.405 \\ &\textbf{\textsc{Wachsmuth$_{All}$}}  &0.313 &0.215 &0.290 &0.320 &0.097 &0.223 &0.453 &0.169 &0.332 \\
&\textbf{\textsc{Wachsmuth$_{CFS}$}} &0.543 &0.326 &0.476 &0.549 &0.192 &0.399 &0.524 &0.261 &0.432 \\
&\textbf{\textsc{SVR$_{tfidf}$}} &0.466 &0.364 &0.457 &0.292 &0.153 &0.247 &0.435 &0.345 &0.452 \\
&\textbf{\textsc{SVR$_{embd}$}}&0.411 &0.278 &0.379 &0.393 &0.096 &0.258 &0.205 &0.191 &0.234 \\
&\textbf{\textsc{BERT ST}} &\textbf{0.696} &\textbf{0.512} &\textbf{0.665} &0.544 &0.222 &0.418 &\textbf{0.556} &0.484 &0.609 \\
&\textbf{\textsc{BERT MT$_{flat}$}} &0.672 &0.499 &0.644 &\textbf{0.587} &0.273 &\textbf{0.473} &0.550 &\textbf{0.489} &0.610 \\
&\textbf{\textbf{\textsc{BERT MT$_{hier}$}}}  &0.660 &0.478 &0.626 &0.445 &\textbf{0.280} &0.408 &0.555 &0.488 &\textbf{0.611} \\
\bottomrule
\end{tabular}
\caption{Pearson correlations of our model predictions with the annotation scores for the four argument quality dimensions on the three different test annotations for three domains when training on the domain-specific data only. We compare with the best result of the in-domain setting. Numbers in bold indicate best performances.}\label{tbl:in-domains}
\end{table*}
%
%
%

\jttodo{A few things: 1. the table is massive. How would you shorten it?  2. can we make a general remark about performance here?  Like, are these numbers good?  How do they compare to argumentation type scores? What do you mean by "argumentation type scores"?}
Similar to the inter-annotator agreement, the performances achieved vary across the domains even for single argument quality dimensions: On the \emph{Expert} test set of the debate forums domain the best model, \textsc{BERT MT$_{hier}$}, achieves a correlation coefficient with the annotation scores for reasonableness of $.280$ and on the QA forums \emph{Crowd} test set the best model, \textsc{BERT ST}, achieves a performance of $.696$. Except for a single case, the BERT-based models are able to outperform the other methods. Overall, the best method seems to be \textsc{BERT MT$_{flat}$}, which outperforms the other methods in $19$ out of $35$ cases, followed by \textsc{BERT ST} and \textsc{BERT MT$_{hier}$}, which are best in $8$ and $7$ cases, respectively. %%% write about the new baseline
Note, that the Pearson correlation score of \textsc{Arg Length} is relatively high across all domains and properties and typically outperforms the simple SVR-based baselines, which indicates a slight bias in the data set. This is not surprising given that \corpus contains real-word texts varying in length and often, a longer argument contains more useful information. However, the proposed models still able to outperform this baseline by a large margin which demonstrates their ability to capture useful information. Interestingly, the delta between what the BERT-based model performances and the \textsc{Arg Length} baseline is even higher on the \emph{Expert}-annotated test set than for the crowd.
This might reflect that our linguistic expert annotators are much more able to abstract from plain amount of information to actual argumentative quality aspects.
%
%
% TRAINING ON ALL DOMAINS
%


Next,\jttodo{I would make this its own subsection -- What would be an appropriate name? I am not sure with this.} we evaluate our models when trained not only on the domain-specific data, i.e., \emph{in-domain}, but on the joint training set covering all domains. The respective results for the four argument quality dimensions on the six different domain-specific test sets can be seen in Table \ref{tbl:all-domains}. We compare with the best in-domain model.
\setlength{\tabcolsep}{4pt}
\begin{table*}[!t]\centering
%\scriptsize
\small
\begin{tabular}{llrrrrrrrrrr}\toprule
&\textbf{} &\multicolumn{3}{c}{\textbf{QA forums}} &\multicolumn{3}{c}{\textbf{Debate Forums}} &\multicolumn{3}{c}{\textbf{Review Forums}} \\\cmidrule{3-11}
&\textbf{Model} &\textbf{Crowd} &\textbf{Expert} &\textbf{Mix} &\textbf{Crowd} &\textbf{Expert} &\textbf{Mix} &\textbf{Crowd} &\textbf{Expert} &\textbf{Mix} \\\midrule
\multirow{6}{*}{\textbf{Overall}} &\textbf{Best in-domain} &0.681 &\textbf{0.535} &0.667 &\textbf{0.607} &0.362 &0.537 &0.619 &0.478 &0.605 \\
&\textbf{\textsc{SVR$_{tfidf}$}} &0.407 &0.280 &0.379 &0.202 &0.109 &0.171 &0.570 &0.384 &0.540 \\
&\textbf{\textsc{SVR$_{embd}$}} &0.382 &0.244 &0.346 &0.388 &0.187 &0.314 &0.271 &0.136 &0.224 \\
&\textbf{\textsc{BERT ST}} &0.693 &0.530 &0.676 &0.571 &0.401 &0.545 &0.650 &0.409 &0.596 \\
&\textbf{\textsc{BERT MT$_{flat}$}}  &\textbf{0.697} &\textbf{0.535} &\textbf{0.681} &0.574 &\textbf{0.425} &\textbf{0.562} &\textbf{0.678} &0.443 &\textbf{0.633} \\
&\textbf{\textsc{BERT MT$_{hier}$}}  &0.680 &0.522 &0.665 &0.576 &0.424 &\textbf{0.562} &0.618 &\textbf{0.469} &0.622 \\
\midrule
\multirow{6}{*}{\textbf{Cogency}} &\textbf{Best in-domain} &0.651 &0.468 &\textbf{0.638} &\textbf{0.622} &0.353 &0.541 &\textbf{0.618} &0.440 &0.561 \\
&\textbf{\textsc{SVR$_{tfidf}$}} &0.374 &0.244 &0.353 &0.164 &0.184 &0.205 &0.532 &0.363 &0.511 \\
&\textbf{\textsc{SVR$_{embd}$}} &0.337 &0.171 &0.292 &0.323 &0.149 &0.261 &0.292 &-0.020 &0.143 \\
&\textbf{\textsc{BERT ST}} &0.639 &0.426 &0.608 &0.540 &0.367 &0.515 &0.601 &0.386 &0.563 \\
&\textbf{\textsc{BERT MT$_{flat}$}}  &\textbf{0.673} &\textbf{0.472} &0.653 &0.560 &0.392 &0.542 &0.610 &0.391 &0.570 \\
&\textbf{\textsc{BERT MT$_{hier}$}}  &0.662 &0.455 &\textbf{0.638} &0.573 &\textbf{0.397} &\textbf{0.552} &0.577 &\textbf{0.465} &\textbf{0.599} \\
\midrule
\multirow{6}{*}{\textbf{Effectiveness}} &\textbf{Best in-domain} &0.656 &0.552 &0.671 &\textbf{0.599} &0.443 &0.570 &0.639 &0.389 &0.555 \\
&\textbf{\textsc{SVR$_{tfidf}$}} &0.381 &0.264 &0.356 &0.258 &0.114 &0.204 &0.506 &0.293 &0.440 \\
&\textbf{\textsc{SVR$_{embd}$}} &0.346 &0.254 &0.331 &0.385 &0.199 &0.324 &0.245 &0.088 &0.175 \\
&\textbf{\textsc{BERT ST}} &0.664 &\textbf{0.574} &\textbf{0.686} &0.544 &\textbf{0.492} &\textbf{0.598} &\textbf{0.711} &0.387 &0.601 \\
&\textbf{\textsc{BERT MT$_{flat}$}}  &\textbf{0.676} &0.536 &0.670 &0.569 &0.444 &0.578 &0.683 &\textbf{0.409} &\textbf{0.603} \\
&\textbf{\textsc{BERT MT$_{hier}$}} &0.657 &0.523 &0.653 &0.573 &0.462 &0.592 &0.644 &0.396 &0.576 \\
\midrule
\multirow{6}{*}{\textbf{Reasonableness}} &\textbf{Best in-domain} &\textbf{0.696} &\textbf{0.512} &\textbf{0.665} &\textbf{0.587} &0.280 &0.473 &0.556 &\textbf{0.489} &0.611 \\
&\textbf{\textsc{SVR$_{tfidf}$}} &0.451 &0.345 &0.438 &0.240 &0.118 &0.198 &0.599 &0.422 &0.584 \\
&\textbf{\textsc{SVR$_{embd}$}} &0.486 &0.297 &0.430 &0.392 &0.189 &0.321 &0.283 &0.182 &0.263 \\
&\textbf{\textsc{BERT ST}} &0.658 &0.495 &0.635 &0.550 &0.320 &\textbf{0.487} &0.616 &0.437 &0.603 \\
&\textbf{\textsc{BERT MT$_{flat}$}}  &0.691 &0.503 &0.657 &0.538 &\textbf{0.328} &0.486 &\textbf{0.667} &0.443 &0.631 \\
&\textbf{\textbf{\textsc{BERT MT$_{hier}$}}} &0.665 &0.485 &0.633 &0.554 &0.312 &0.483 &0.642 &0.476 &\textbf{0.643} \\
\bottomrule
\end{tabular}
\caption{Pearson correlations of the model predictions with the annotation scores for the four argument quality dimensions on the three different test annotations for three domains when training on the joint training sets of all domains. We compare with the best result of the in-domain setting. Numbers in bold indicate best performances.}\label{tbl:all-domains}
\end{table*}
%
%
%
As it can be seen from the table, in $25$ out of $36$ cases training on all domains increases the performance compared to the best in-domain model ($69 \%$ of the cases). While the models are less domain-specific, the increased amount of data leads to better convergence. Especially on the \emph{Expert} test set of the debate forums, and the \emph{Crowd} test set of the review forums, the gains can be high -- up to $11$ percentage points! \cntodo{we should have more analysis of these results before getting into the experiments on other datasets}
%
%
%
\subsection{Experiments on Dagstuhl-15512-ArgQuality-Corpus-v2}
We report on our experiments employing Dagstuhl-15512-ArgQuality-Corpus-v2.
\paragraph{Experimental Setup.}
%% Data
The Dagstuhl-ArgQuality-Corpus\footnote{\url{http://argumentation.bplaced.net/arguana/data}}~\cite{wachsmuth-etal-2017-computational} was presented in combination with the taxonomy of argument quality described above and consists of $320$ web debate arguments annotated with all $15$ argument quality aspects. The arguments were originally taken from UKPConvArgRank~\cite{habernal-gurevych-2016-argument}.
% Trained models
Again, we take the \textsc{BERT MT$_{Flat}$} models trained either \emph{in-domain} or \emph{all-domain} on the \corpus and predict on the whole corpus. In order to obtain a single score per annotation instance and dimension, we apply two ways of aggregating the annotations provided by the authors: (1) majority vote, and (2) mean aggregation. We compare with the human performance, which we obtain by macro averaging the correlations we get when comparing individual annotators to the aggregated score (to which they contributed).% I cannot just take kappa here right?

\paragraph{Results.} 
%
%
%
%
\begin{comment}
%
%
% THIS TABLE IS COMMENTED AS WE ARE SQEEZING IT NEXT TO THE OTHER TABLE
\begin{table}[t]\centering
\small
\begin{tabular}{lrrrrrr}\toprule
\textbf{} &\textbf{} &\multicolumn{2}{c}{\textbf{Majority}} &\multicolumn{2}{c}{\textbf{Mean}} \\\cmidrule{3-6}
\textbf{Domain} &\textbf{Dimension} &\textbf{$r$} &\textbf{$\rho$} &\textbf{$r$} &\textbf{$\rho$} \\\midrule
All &Overall &\textbf{0.454} &\textbf{0.453} &\textbf{0.515} &\textbf{0.502} \\
&Cogency &0.382 &0.383 &0.443 &0.428 \\
&Effectiveness &0.406 &0.397 &0.478 &0.466 \\
&Reasonableness &0.427 &0.396 &0.492 &0.456 \\
\midrule
QA forums &Overall &\textbf{0.425} &\textbf{0.424} &\textbf{0.475} &\textbf{0.473} \\
&Cogency &0.344 &0.343 &0.419 &0.407 \\
&Effectiveness &0.369 &0.369 &0.453 &0.454 \\
&Reasonableness &0.408 &0.393 &0.467 &0.447 \\
\midrule
Debate forums &Overall &0.365 &0.347 &0.423 &0.402 \\
&Cogency &0.306 &0.294 &0.364 &0.344 \\
&Effectiveness &0.338 &0.326 &0.419 &\textbf{0.404} \\
&Reasonableness &\textbf{0.398} &\textbf{0.355} &\textbf{0.431} &0.389 \\
\midrule
Review forums &Overall &0.315 &\textbf{0.312} &\textbf{0.346} &\textbf{0.335} \\
&Cogency &0.284 &0.276 &0.307 &0.302 \\
&Effectiveness &0.257 &0.260 &0.300 &0.303 \\
&Reasonableness &\textbf{0.325} &0.309 &0.338 &0.317 \\
\bottomrule
\end{tabular}
\caption{Pearson and Spearman correlation coefficients when predicting with our \textsc{BERT MT$_{Flat}$} trained \emph{all-domain} or \emph{in-domain} on the Dagstuhl data. We correlate our prediction for each dimension with its associated true label when applying mean or majority aggregation on the annotations.}\label{tab:dagstuhl}
\end{table}
\end{comment}


\begin{table}
\parbox{.49\linewidth}{
\centering
\scriptsize
\begin{tabular}{llcccc}\toprule
\textbf{} &\textbf{} &\multicolumn{2}{c}{\textbf{WA}} &\multicolumn{2}{c}{\textbf{MACE-P}} \\\cmidrule{3-6}
\textbf{Domain} &\textbf{Dimension} &\textbf{$r$} &\textbf{$\rho$} &\textbf{$r$} &\textbf{$\rho$} \\\midrule
\textsc{BERT IBM} & -- & 0.492 &	0.456	& 0.503	 & 0.493 \\
\newcite{gretz2019large} & -- & 0.52 & 0.48 &	0.53 & 0.52\\
\midrule
All &Overall &\textbf{0.313} &\textbf{0.303} &\textbf{0.325} &\textbf{0.322} \\
&Cogency &0.311 &0.300 &0.322 &0.318 \\
&Effectiveness &\textbf{0.313} &\textbf{0.303} &\textbf{0.325} &\textbf{0.322} \\
&Reasonableness &0.304 &0.298 &0.317 &0.316 \\
\midrule
QA Forums &Overall &0.258 &0.224 &0.260 &0.242 \\
&Cogency &\textbf{0.269} &\textbf{0.228} &\textbf{0.271} &\textbf{0.247} \\
&Effectiveness &0.262 &0.225 &0.264 &0.243 \\
&Reasonableness &0.262 &0.226 &0.265 &0.244 \\
\midrule
Debate Forums &Overall &\textbf{0.336} &\textbf{0.326} &0.359 &0.348 \\
&Cogency &0.331 &0.321 &0.354 &0.343 \\
&Effectiveness &\textbf{0.336} &\textbf{0.326} &\textbf{0.360} &\textbf{0.349} \\
&Reasonableness &0.333 &0.319 &0.355 &0.340 \\
\midrule
Review Forums &Overall &0.150 &0.145 &0.162 &0.157 \\
&Cogency &0.139 &0.138 &0.155 &0.149 \\
&Effectiveness &\textbf{0.152} &\textbf{0.151} &\textbf{0.165} &\textbf{0.161} \\
&Reasonableness &0.149 &0.148 &0.165 &0.160 \\
\bottomrule
\end{tabular}
\caption{Performances of the \textsc{BERT MT$_{Flat}$} models trained on varying domains of the \corpus when predicting on IBM-Rank-30k either evaluated against the weighted average score (WA) or the MACE-based aggregation score (MACE-P). We report the Pearson ($r$) and the Spearman correlation coefficient (\textbf{$\rho$}). Scores in bold indicate best performances.}\label{tbl:ibm-predict-results}
}
\hfill
\parbox{.49\linewidth}{
\centering
%
\scriptsize
\begin{tabular}{llrrrrr}\toprule
\textbf{} &\textbf{} &\multicolumn{2}{c}{\textbf{Majority}} &\multicolumn{2}{c}{\textbf{Mean}} \\\cmidrule{3-6}
\textbf{Domain} &\textbf{Dimension} &\textbf{$r$} &\textbf{$\rho$} &\textbf{$r$} &\textbf{$\rho$} \\\midrule
All &Overall &\textbf{0.454} &\textbf{0.453} &\textbf{0.515} &\textbf{0.502} \\
&Cogency &0.382 &0.383 &0.443 &0.428 \\
&Effectiveness &0.406 &0.397 &0.478 &0.466 \\
&Reasonableness &0.427 &0.396 &0.492 &0.456 \\
\midrule
QA forums &Overall &\textbf{0.425} &\textbf{0.424} &\textbf{0.475} &\textbf{0.473} \\
&Cogency &0.344 &0.343 &0.419 &0.407 \\
&Effectiveness &0.369 &0.369 &0.453 &0.454 \\
&Reasonableness &0.408 &0.393 &0.467 &0.447 \\
\midrule
Debate forums &Overall &0.365 &0.347 &0.423 &0.402 \\
&Cogency &0.306 &0.294 &0.364 &0.344 \\
&Effectiveness &0.338 &0.326 &0.419 &\textbf{0.404} \\
&Reasonableness &\textbf{0.398} &\textbf{0.355} &\textbf{0.431} &0.389 \\
\midrule
Review forums &Overall &0.315 &\textbf{0.312} &\textbf{0.346} &\textbf{0.335} \\
&Cogency &0.284 &0.276 &0.307 &0.302 \\
&Effectiveness &0.257 &0.260 &0.300 &0.303 \\
&Reasonableness &\textbf{0.325} &0.309 &0.338 &0.317 \\
\bottomrule
\end{tabular}
\caption{Pearson ($r$) and Spearman ($\rho)$ correlation coefficients when predicting with our \textsc{BERT MT$_{Flat}$} trained \emph{all-domain} or \emph{in-domain} on the Dagstuhl data. We correlate our prediction for each dimension with its associated true label when applying mean or majority aggregation on the annotations. Scores in bold indicate best performances per domain.}\label{tab:dagstuhl}
}
\end{table}

Training on our joint training set across all domains yields the highest correlation scores and generally, the annotations related to overall argument quality and reasonableness correlate best with our scores. To the best of our knowledge, we are the first to have a trained model in-place which is able to predict scores for fine-grained argument quality dimensions.
\cntodo{the Dagstuhl and IBM experiments feel tacked on. we need to motivate them better (and work on organization---that may help too}
%
%
\section{Synergies between practical and theory-based AQ approaches: Experiments on IBM-Rank-30k}
In order to investigate potential synergies between practical and theory-based computation AQ assessment approaches, we next conduct a bi-directional experiment. To this end, we employ the recently presented IBM-Rank-30k \cite{gretz2019large}.\jttodo{we need to write the motivation for doing this}\cntodo{these should also be anin their own section}
\paragraph{Experimental Setup.}
% Data
IBM-Rank-30k consists of in total 30,497 arguments
from 280 contributors. Each argument is restricted to a minimum of 35 and a maximum of 210 characters. The arguments relate to $71$ topics, which are split into a training set consisting of $49$ topics, a development set consisting of $7$ topics, and a test set consisting of $15$ topics. Manual inspection of individual instances revealed that the nature of the texts differs from each of the domains covered in \corpus a lot. %% histogram of distributions?
\jttodo{in what ways does it differ?}
% Trained models
We take the \textsc{BERT MT$_{Flat}$} models trained on varying domains of the \corpus and predict on the test portion of IBM-ArgRank-30k. This way, we obtain an idea about (1) which domain, and (2) which dimension is closest to the data and annotations in IBM-ArgRank-30k.  
% Baselines
We compare against the best score reported in the original paper as well as against our own replication/reproduction using BERT$_{BASE}$, dubbed \textsc{BERT IBM}.\footnote{Note that \newcite{gretz2019large} do not indicate whether they employ BERT$_{BASE}$ or BERT$_{LARGE}$.} \jttodo{just so it's clear, they made their own BERT model for their data and we tried our best to reproduce it so we could have something that runs on both our data and theirs?  How is their model different than our BERT?  Also, did you email Gretz et al.?  We should do so if we don't get called out for accidentally comparing to the wrong BERT}
%%% Shall we actually do that? Right now I have the feeling that this does not give us much insight, except that there is a drop in performance as expected
% Optimization
We optimize the \textsc{BERT IBM} baseline by grid searching for the learning rate $\lambda \in \{2e-5, 3e-5\}$ and the number of training epochs $\in \{3,4\}$ on the development set portion of IBM-Rank-30k.
For the already trained models from Section .. , no optimization is necessary.
\paragraph{Results.} The results of our experiments using  IBM-Rank-30k are given in Table \ref{tbl:ibm-predict-results}. We report the Pearson ($r$) and the Spearman correlation coefficients (\textbf{$\rho$}) against the weighted average annotation (WA) and the MACE-based aggregation given in the data set.
%
%
%
%
%
\begin{comment}
% THIS TABLE IS COMMENTED AS WE ARE SQEEZING IT NEXT TO THE OTHER TABLE
\begin{table}[t!]\centering
\small
\begin{tabular}{llcccc}\toprule
\textbf{} &\textbf{} &\multicolumn{2}{c}{\textbf{WA}} &\multicolumn{2}{c}{\textbf{MACE-P}} \\\cmidrule{3-6}
\textbf{Domain} &\textbf{Dimension} &\textbf{$r$} &\textbf{$\rho$} &\textbf{$r$} &\textbf{$\rho$} \\\midrule
All &Overall &\textbf{0.313} &\textbf{0.303} &\textbf{0.325} &\textbf{0.322} \\
&Cogency &0.311 &0.300 &0.322 &0.318 \\
&Effectiveness &\textbf{0.313} &\textbf{0.303} &\textbf{0.325} &\textbf{0.322} \\
&Reasonableness &0.304 &0.298 &0.317 &0.316 \\
QA Forums &Overall &0.258 &0.224 &0.260 &0.242 \\
&Cogency &\textbf{0.269} &\textbf{0.228} &\textbf{0.271} &\textbf{0.247} \\
&Effectiveness &0.262 &0.225 &0.264 &0.243 \\
&Reasonableness &0.262 &0.226 &0.265 &0.244 \\
Debate Forums &Overall &\textbf{0.336} &\textbf{0.326} &0.359 &0.348 \\
&Cogency &0.331 &0.321 &0.354 &0.343 \\
&Effectiveness &\textbf{0.336} &\textbf{0.326} &\textbf{0.360} &\textbf{0.349} \\
&Reasonableness &0.333 &0.319 &0.355 &0.340 \\
Review Forums &Overall &0.150 &0.145 &0.162 &0.157 \\
&Cogency &0.139 &0.138 &0.155 &0.149 \\
&Effectiveness &\textbf{0.152} &\textbf{0.151} &\textbf{0.165} &\textbf{0.161} \\
&Reasonableness &0.149 &0.148 &0.165 &0.160 \\
\bottomrule
\end{tabular}
\caption{Performances of the \textsc{BERT MT$_{Flat}$} models trained on varying domains of the \corpus when predicting on IBM-Rank-30k either evaluated against the weighted average score (WA) or the MACE-based aggregation score (MACE-P). We report the Pearson ($r$) and the Spearman correlation coefficient (\textbf{$\rho$}). Scores in bold indicate best performances.}\label{tbl:ibm-predict-results}
\end{table}
%
%
\end{comment}
%
%
% Analysis

\jttodo{the next two paragraphs got very dense.  I'll need to re-read}
As expected, the zero-shot domain transfer results in a large drop compared to training on the associated train set of IBM-ArgRank-30k. However, quite surprisingly, the model trained on the debate forums reaches the highest correlation scores -- even higher than the model trained on \emph{all-domains}. Further, in most cases, the effectiveness predictions correlate best with the annotations provided by \newcite{gretz2019large}. This is in-line with the authors' obervations.
% Data contains many "arguments", which are more premises than actual arguments
%
%

In order to validate these findings we perform the experiment vice versa: We (1) train a BERT-base regressor as defined in Equation \ref{eq:PredictionT} on the MACE-P annotations of IBM-ArgRank-30k, which corresponds to our \textsc{BERT IBM} baseline from before. Then, we predict on \corpus and correlatate the resulting scores with our annotations for the four argument quality dimensions on each of our three test sets per domain. Additionally, we (2) draw inspiration from \newcite{phang_stilts} and use IBM-ArgRank-30k in the Supplementary Training on Intermediate Labeled Tasks-setup (STILT). That is, we take the trained encoder from (1) and continue training the model as \textsc{BERT IBM MT$_{flat}$} in the all-domain setup.
We compare both models with the \textsc{BERT MT$_{flat}$} from Table \ref{tbl:all-domains}.
%
%
%
\begin{table}[!t]\centering
\small
\begin{tabular}{llrrrrrrrrrr}\toprule
& &\multicolumn{3}{c}{\textbf{QA forums}} &\multicolumn{3}{c}{\textbf{Debate Forums}} &\multicolumn{3}{c}{\textbf{Review Forums}} \\\cmidrule{3-11}
& &\textbf{Crowd} &\textbf{Expert} &\textbf{Mix} &\textbf{Crowd} &\textbf{Expert} &\textbf{Mix} &\textbf{Crowd} &\textbf{Expert} &\textbf{Mix} \\\midrule
\multirow{3}{*}{\textbf{Overall}} &\textsc{BERT IBM} &0.362 &0.348 &0.392 &0.304 &0.254 &0.317 &0.250 &0.048 &0.154 \\
&\textsc{BERT IBM MT$_{flat}$} &0.669 &\textbf{0.536} &0.666 &0.536 &\textbf{0.425} &0.543 &0.625 &0.386 &0.568 \\
&\textsc{BERT MT$_{flat}$} &\textbf{0.697} &0.535 &\textbf{0.681} &\textbf{0.574} &\textbf{0.425} &\textbf{0.562} &\textbf{0.678} &\textbf{0.443} &\textbf{0.633} \\
\midrule
\multirow{3}{*}{\textbf{Cogency}} &\textsc{BERT IBM}&0.350 &0.297 &0.368 &0.292 &0.192 &0.274 &0.218 &0.053 &0.149 \\
&\textsc{BERT IBM MT$_{flat}$} &0.654 &0.465 &0.639 &0.526 &0.381 &0.518 &0.566 &0.381 &0.541 \\
&\textsc{BERT MT$_{flat}$} &\textbf{0.673} &\textbf{0.472} &\textbf{0.653} &\textbf{0.560} &\textbf{0.392} &\textbf{0.542} &\textbf{0.610} &\textbf{0.391} &\textbf{0.570} \\
\midrule
\multirow{3}{*}{\textbf{Effectiveness}} &\textsc{BERT IBM} &0.378 &0.387 &0.426 &0.314 &0.334 &0.378 &0.321 &0.064 &0.195 \\
&\textsc{BERT IBM MT$_{flat}$} &0.671 &\textbf{0.553} &\textbf{0.678} &0.551 &\textbf{0.481} &\textbf{0.594} &0.639 &0.356 &0.545 \\
&\textsc{BERT MT$_{flat}$} &\textbf{0.676} &0.536 &0.670 &\textbf{0.569} &0.444 &0.578 &\textbf{0.683} &\textbf{0.409} &\textbf{0.603} \\
\midrule
\multirow{3}{*}{\textbf{Reasonableness}} &\textsc{BERT IBM} &0.354 &0.278 &0.348 &0.287 &0.155 &0.246 &0.216 &0.070 &0.151 \\
&\textsc{BERT IBM MT$_{flat}$} &0.670 &0.487 &0.637 &0.515 &0.314 &0.465 &0.652 &0.384 &0.581 \\
&\textsc{BERT MT$_{flat}$} &\textbf{0.691} &\textbf{0.503} &\textbf{0.657} &\textbf{0.538} &\textbf{0.328} &\textbf{0.486} &\textbf{0.667} &\textbf{0.443} &\textbf{0.631} \\
\bottomrule
\end{tabular}
\caption{Pearson correlations on \corpus when predicting with \textsc{BERT IBM} (trained on IBM-Rank-30k) and \textsc{BERT IBM MT$_{flat}$} trained on IBM-Rank-30k in STILT setup fine-tuned on \corpus in comparison to \textsc{BERT MT$_{flat}$}.}\label{tbl:stilt}
\end{table}
%
%
%
%
The results are listed in Table~\ref{tbl:stilt}. Again: as expected, the zero-shot domain transfer using \textsc{BERT IBM} results in a huge loss in performance compared to \textsc{BERT MT$_{flat}$}. However, when reusing the enconder in the STILT setup, \textsc{BERT IBM MT$_{flat}$}, the losses can be flattended out -- in some cases even ourperforming \textsc{BERT MT$_{flat}$}. This is especially the case when correlating the predictions with our annotations for the effectiveness dimensions. 

All in all, the findings of our bi-directional experiment on IBM, i.e, the facts that automatic predictions (1) in the first case, obtained by a theory-based AQ-informed model on a large (practical) AQ data set, correlate mostly with the effectiveness dimension, and
(2) in the second case, the transferred knowledge in \textsc{BERT IBM MT$_{flat}$} seems to help most for the effectiveness dimension the hypothesis in an additionally conducted manual annotation study on a s obtained , that  mostly captured effectiveness in their annotation study. suggest two simple ways, how one the one hand, a theory-based approach can practical AQ research and increase interpretability of research outcomes and, on the other hand, help to increase the efficacy of theory-based AQ models when interested in a certain domain and dimension.
%
